Parameter-Saving Adversarial Training: Reinforcing Multi-Perturbation Robustness via Hypernetworks

Adversarial training serves as one of the most popular and effective methods to defend against adversarial perturbations. However, most defense mechanisms only consider a single type of perturbation while various attack methods might be adopted to perform stronger adversarial attacks against the deployed model in real-world scenarios, e.g., $\ell_2$ or $\ell_\infty$. Defending against various attacks can be a challenging problem since multi-perturbation adversarial training and its variants only achieve suboptimal robustness trade-offs, due to the theoretical limit to multi-perturbation robustness for a single model. Besides, it is impractical to deploy large models in some storage-efficient scenarios. To settle down these drawbacks, in this paper we propose a novel multi-perturbation adversarial training framework, parameter-saving adversarial training (PSAT), to reinforce multi-perturbation robustness with an advantageous side effect of saving parameters, which leverages hypernetworks to train specialized models against a single perturbation and aggregate these specialized models to defend against multiple perturbations. Eventually, we extensively evaluate and compare our proposed method with state-of-the-art single/multi-perturbation robust methods against various latest attack methods on different datasets, showing the robustness superiority and parameter efficiency of our proposed method, e.g., for the CIFAR-10 dataset with ResNet-50 as the backbone, PSAT saves approximately 80\% of parameters with achieving the state-of-the-art robustness trade-off accuracy.

==> figs/fig_testing.tex <==
%%变量
\newcommand{\xBias}{0}
\newcommand{\yBias}{0}
\newcommand{\xxBias}{0}
\newcommand{\yyBias}{0}
\newcommand{\scaling}{0}

%%函数
%多边形
\newcommand{\arrowWidth}{0.04cm}
\newcommand{\mypolygon}[8]{
%{#1:x}{#2:y}{#3:h}{#4:l}{#5:w}{#6:color}{#7:opacity}{#8:rounded corners}
    \draw[#6!100, fill=#6!#7, #8] (#1-0.5*#4,#2) -- (#1+0.5*#4,#2) -- (#1+0.5*#5,#2+#3) -- (#1-0.5*#5,#2+#3) -- (#1-0.5*#4,#2);
}

%长方体
\newcommand{\mycuboid}[9]{
%{#1:Ox}{#2:Oy}{#3:Oz}{#4:l}{#5:w}{#6:h}{#7:color}{#8:line opacity}{#9:fill opacity}
\coordinate (O) at (#1,#2,#3);
\coordinate (A) at (#1,#2,#3+#6);
\coordinate (B) at (#1+#4,#2,#3+#6);
\coordinate (C) at (#1+#4,#2,#3);
\coordinate (D) at (#1,#2+#5,#3);
\coordinate (E) at (#1,#2+#5,#3+#6);
\coordinate (F) at (#1+#4,#2+#5,#3+#6);
\coordinate (G) at (#1+#4,#2+#5,#3);
\draw[#7!#8,fill=#7!#9] (O) -- (A) -- (B) -- (C) -- cycle;% Front Face
\draw[#7!#8,fill=#7!#9] (O) -- (A) -- (E) -- (D) -- cycle;% Left Face
\draw[#7!#8,fill=#7!#9] (O) -- (C) -- (G) -- (D) -- cycle;% Bottom Face
\draw[#7!#8,fill=#7!#9] (D) -- (E) -- (F) -- (G) -- cycle;% Back Face
\draw[#7!#8,fill=#7!#9] (B) -- (C) -- (G) -- (F) -- cycle;% Right Face
\draw[#7!#8,fill=#7!#9] (A) -- (B) -- (F) -- (E) -- cycle;% Top Face
}
%------------------------------------------------------------------------

\renewcommand{\xBias}{15}
\renewcommand{\yBias}{-1.5}
\mypolygon{14+\xBias}{4+\yBias}{1.5}{6}{4}{gray}{70}{};
\node at (14+\xBias,4+1.5*0.5+\yBias) {Layer $1$};
\mypolygon{14+\xBias}{5.6+\yBias}{1.2}{3.9}{2.4}{gray}{70}{};
\node at (14+\xBias,5.6+1.2/2+\yBias) {$\vdots$};
\mypolygon{14+\xBias}{6.9+\yBias}{1}{2.3}{1}{gray}{70}{};
\node at (14+\xBias,6.9+1/2+\yBias) {Layer $l$};
\draw[->,line width=\arrowWidth] (14+\xBias,7.9+\yBias) -- (14+\xBias,9+\yBias);
\node at (7+\xBias,2.8+0.6+\yBias) {\includegraphics[width=3cm,height=2cm]{figs/cat_noised.png}};
\node at (7+\xBias,1.5+0.6+\yBias) {Test Data $x_t$};
\draw[->,line width=\arrowWidth] (7+1.55+\xBias,2.8+0.6+\yBias) -- ++(5.5,0) -- +(0,0.6);
\mypolygon{14+\xBias}{9+\yBias}{1}{3}{3}{green}{20}{rounded corners};
\node at (14+\xBias,9+1/2+\yBias) {\begin{tabular}{c}Output Ensemble\\$Y=\bigcup\{y_p\}$\end{tabular}};
\draw[->,line width=\arrowWidth] (14-3/2+\xBias,9+1/2+\yBias) -- +(-1.2,0);
\mypolygon{14-3/2-1.2-2.8/2+\xBias}{9+\yBias}{1}{2.8}{2.8}{green}{80}{rounded corners};
\node at (14-3/2-1.2-2.8/2+\xBias,9+1/2+\yBias) {\begin{tabular}{c}Lowest-Entropy\\Stragety\end{tabular}};
\draw[->,line width=\arrowWidth] (14-3/2-1.2-2.8+\xBias,9+1/2+\yBias) -- +(-1,0);
\node at (14-3/2-1.2-2.8-1-1.4+\xBias,9+1/2+\yBias)[scale=1.1]{\begin{tabular}{c}\textbf{Final Output}\\$\mathbf{y_\mathrm{final}}$\end{tabular}};

\mypolygon{6.3+\xBias}{5+\yBias}{1.8}{5}{5}{gray}{70}{rounded corners};
\node at (6.3+\xBias,5+1.8/2+\yBias) {
\begin{tabular}{c}
     \textbf{Hypernetworks Ensemble} \\
     $\mathbf{\mathcal{F}_\mathcal{H}=\bigcup_{p\in \mathcal{A}}\{z_p,\mathcal{H}_p\}}$
\end{tabular}
};

\draw[->,line width=\arrowWidth] (8.8+\xBias,6.6+\yBias) -- ++(1.5,0) -- ++(0,0.75) -- ++(2.8,0);
\node at (8.8+1.5+2.8/2+\xBias,6.6+0.75+0.3+\yBias) {$\theta^l_p$};
\draw[->,line width=\arrowWidth] (8.8+\xBias,5.9+\yBias) -- ++(1.5,0) -- ++(0,0.5) -- ++(2.2,0);
\node at (8.8+1.5+2.2/2+\xBias,5.9+0.5+0.3+\yBias/2++\yBias/2) {$\vdots$};
\draw[->,line width=\arrowWidth] (8.8+\xBias,5.3+\yBias) -- ++(1.5,0) -- ++(0,-0.5) -- ++(1.2,0);
\node at (8.8+1.5+1.2/2+\xBias,5.3-0.5+0.3+\yBias) {$\theta^1_p$};
